Population based change-point detection for the identification of homozygosity islands

In this paper, we propose a new method for offline change-point detection on some parameters of the distribution of a random vector. We introduce a penalized maximum likelihood approach that can be efficiently computed by a dynamic programming algorithm or approximated by a fast greedy binary splitting algorithm. We prove both algorithms converge almost surely to the set of change-points under very general assumptions on the distribution and independent sampling of the random vector. In particular, we show the assumptions leading to the consistency of the algorithms are satisfied by categorical and Gaussian random variables. This new approach is motivated by the problem of identifying homozygosity islands on the genome of individuals in a population. Our method directly tackles the issue of identification of the homozygosity islands at the population level, without the need of analyzing single individuals and then combining the results, as is made nowadays in state-of-the-art approaches.

==> Configurations/Macros.tex <==
%%% Operators %%%

\DeclareMathOperator*{\argmax}{\textup{argmax}}
\DeclareMathOperator*{\argmin}{\textup{argmin}}
%%%

%%% Math enviroments %%%

\theoremstyle{definition}
%\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}

%\theoremstyle{theorem}
%\newtheorem{theorem}{Theorem}

%\theoremstyle{definition}
%\newtheorem{lem}[theo]{Lemma}

%\theoremstyle{definition}
%\newtheorem{prop}[theo]{Proposition}

%\theoremstyle{definition}
%\newtheorem{conj}[theo]{Conjecture}

%%%

%%% pseudocode %%%
\algdef{SE}[VARIABLES]{Variables}{EndVariables}
   {\algorithmicvariables}
   {\algorithmicend\ \algorithmicvariables}
\algnewcommand{\algorithmicvariables}{\textbf{global variables}}

%%% Macros for hat and bar overscript
%% Wide hat
\newcommand\reallywidehat[1]{%
\savestack{\tmpbox}{\stretchto{%
  \scaleto{%
    \scalerel*[\widthof{\ensuremath{#1}}]{\kern-.6pt\bigwedge\kern-.6pt}%
    {\rule[-\textheight/2]{1ex}{\textheight}}%WIDTH-LIMITED BIG WEDGE
  }{\textheight}% 
}{0.5ex}}%
\stackon[1pt]{#1}{\tmpbox}%
}

%% Wide bar
\newcommand\widebar[1]{\ThisStyle{%
  \setbox0=\hbox{$\SavedStyle#1$}%
  \stackengine{.5pt+\LMpt}{$\SavedStyle#1$}{%
    \rule{\wd0}{\dimexpr.3\LMpt+.3pt}%
  }{O}{c}{F}{T}{S}%
}}


\newcommand{\ouset}[3]{ \overset{#3}{\underset{#1}{#2}} }

==> Configurations/Packages.tex <==
% ---------------------------------------------------------------------------- %
% Packages
\usepackage[T1]{fontenc}
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage[pdftex]{graphicx}           % usamos arquivos pdf/png como figuras
\usepackage{subfigure}
\usepackage{setspace}                   % espaçamento flexível
\usepackage{indentfirst}                % indentação do primeiro parágrafo
\usepackage{makeidx}                    % índice remissivo
\usepackage[nottoc]{tocbibind}          % acrescentamos a bibliografia/indice/conteudo no Table of Contents
\usepackage{courier}                    % usa o Adobe Courier no lugar de Computer Modern Typewriter
\usepackage{type1cm}                    % fontes realmente escaláveis
\usepackage{listings}                   % para formatar código-fonte (ex. em Java)
\usepackage{titletoc}
%\usepackage[bf,small,compact]{titlesec} % cabeçalhos dos títulos: menores e compactos
\usepackage[fixlanguage]{babelbib}
\usepackage[font=small,format=plain,labelfont=bf,up,textfont=it,up]{caption}
\usepackage[usenames,svgnames,dvipsnames]{xcolor}
\usepackage[a4paper,top=2.54cm,bottom=2.0cm,left=2.0cm,right=2.54cm]{geometry} % margens
%\usepackage[pdftex,plainpages=false,pdfpagelabels,pagebackref,colorlinks=true,citecolor=black,linkcolor=black,urlcolor=black,filecolor=black,bookmarksopen=true]{hyperref} % links em preto
\usepackage[pdftex,plainpages=false,pdfpagelabels,pagebackref,colorlinks=true,citecolor=DarkGreen,linkcolor=NavyBlue,urlcolor=DarkRed,filecolor=green,bookmarksopen=true]{hyperref} % links coloridos
\usepackage[all]{hypcap} % soluciona o problema com o hyperref e capitulos
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=cyan,
}
\usepackage[square,sort,nonamebreak,comma]{natbib}  % citação bibliográfica alpha (alpha-ime.bst)
\fontsize{60}{62}\usefont{OT1}{cmr}{m}{n}{\selectfont}

%%% Math packages %%%
\usepackage{bbm}
\usepackage{amsmath}					% Para declarar operadores matemáticos (\DeclareMathOperator)
\usepackage{amsthm} 					% Teoremas
\usepackage{amssymb}					% Para definir símbolos relacionais, como '\lesssim'
%\usepackage{amsthm}					    % Para definir teoremas sem numeração (\newtheorem*)
\usepackage{enumerate}
\usepackage{scalerel,stackengine}

%%% pseudocode
\usepackage{algorithm}
\usepackage{algpseudocode}

%%% Drawing packages %%%

\usepackage{graphicx}
\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing,angles,quotes}
\usepackage{caption}
\captionsetup[figure]{font=scriptsize}

==> retired.tex <==
%%% Old DP subsection
\subsection{Dynamic programming segmentation algorithm}

As presented in \citet{auger1989algorithms}, dynamic programming can be used to calculate exactly the 
PL estimator. Under an additive regularization, the function we want to minimize can be written as
\begin{align*}
 -l(C;\bx^n) + \lambda J(n)R(C) 
 &= \sum_{j=1}^{k_C} -\log f_{\widehat\theta_j}\Bigl(x_{(c_{j-1}+1):c_j}^{(i)}\Bigr) + \lambda J(n)\rho(c_{j-1} + 1, c_{j})\\ 
  &=  \sum_{j=1}^{k_C} Q((c_{j-1}+1):c_{j}) \,, 
 \end{align*}
where 
\begin{equation*}
Q((c_{j-1}+1):c_{j}) = -\log f_{\widehat\theta_j}\Bigl(x_{(c_{j-1}+1):c_j}^{(i)}\Bigr) + \lambda J(n)\rho(c_{j-1} + 1, c_{j}) \,.
\end{equation*}

The equation shows that we can completely decouple the loss from different blocks. Let $\mathcal{C}_i$ be the set of all ordered change point sets in $1:i$. Define
\begin{equation*}
F_{k}(i) = \min_{C \, \in \, \mathcal{C}_i, \, k_C = k} \Bigg\{\sum_{j=1}^{k}  Q((c_{j-1}+1):c_{j})\Bigg\}  
\end{equation*} 
as the optimal value for $k$ blocks up to variable $i$. The estimator $\widehat C(\bx^n)$ given by \eqref{hatC} is obtained by computing $F_{k}(m)$ for each possible value of $k$ and then choosing $k$
that minimizes $F_{k}(m)$. But notice that
\begin{equation*}
F_{k}(i) = \underset{c \in (k-1):(i-1)}{\min}\{F_{k-1}(c) + Q((c+1):i)\} \,,
\end{equation*}
which establishes a recursion equation for the values of $F_{k}(i)$, $k$ varying from $1$ to $m$ and $i$ from $k$ to $m$. The values of $F_{1}(i)$ can be directly computed, and then we use the recursion to compute the values until we reach $F_{m}(m)$.

%The dynamic programming segmentation algorithm computes the exact solution in \eqref{hatC}.
%A pseudocode for the implementation of the method is provided by Algorithm 1, assuming we can evaluate $Q$ for any given interval. 

In some applications, it could be useful to restrict the maximal number of change points to some value
$K_{max}  \leq m$. Without any restriction we can specify $K_{max}=m$, the dimension of the random vectors. 
Albeit $m$ is fixed and only $n$ grows, the number of variables $m$ can be very large in some applications, so it is useful to express the complexity in terms of both. 
The dynamic programming segmentation algorithm has storage complexity of $O(m^2)$ and time complexity of $O(K_{max}m^2)$. However, we are assuming that $Q$ have been previously computed for any interval in $1:m$. 
To compute $Q$, we need to compute the maximum likelihood estimators for each block. For most models, this can be done efficiently by computing the sufficient statistics, and then compute the entries of $Q$. For the models presented in Examples~\ref{example_gaussian} and \ref{example_categorical}, the time complexity for computing the sufficient statistics is $T(n, m) = O(nm)$, and then $O(m^2)$ to compute the entries of $Q$. In the case where no sufficient statistics exist, we need to reprocess the data every time, so the complexity to compute $Q$ is $O(nm^3)$.
Hence, the final time complexity of the algorithm is $O(T(n, m) + K_{max}m^2)$. In the general case the algorithm is $O(nm^3)$, and can be very slow for big values of $m$.

% \begin{algorithm}[!htbp]
% \caption{Dynamic programming segmentation algorithm}
% \begin{algorithmic}
% \Procedure{DPS}{$K_{max}$}
%     \State $regLossMat \gets array[0,\ldots,K_{max}][1,\ldots,m]$ \Comment{DP data structure to compute $F$}
%     \State $cpMat \gets array[1,\ldots,K_{max}][1,\ldots,m]$ \Comment{data structure to compute change points}
    
    
%     \State $regLossMin \gets \infty$ \Comment{Global minimum}
%     \State $\hat{k} \gets None$
    
%     \For {$k = 0, \ldots, K_{max}$}
%         \For {$i = k, \ldots, m$}
%             \If {$k = 0$} \Comment{Base cases when there are no change points}
%                 \State $regLossMat[0,i] \gets Q(1:i)$
%                 \State \textbf{continue}
%             \EndIf
            
%             \State $regLoss \gets \infty$ \Comment{regularized loss at current iteration}
%             \For{ $c = (k-1),\ldots,(i-1)$}
%                 \If{$regLoss > regLossMat[k-1,c] + Q((1+c):i)$}
%                     \State $ regLoss \gets regLossMat[k-1,c] + Q((1+c):i)$
%                     \State $bestCP \gets c$
%                 \EndIf
%             \EndFor

%             \State $regLossMat[k, i] \gets regLoss$
%             \State $cpMat[k, i] \gets bestCP$ 
%         \EndFor
        
%         \If{ $regLossMin > regLossMat[k, m]$} \Comment{Update number of change points}
%             \State $regLossMin \gets regLossMat[k, m]$
%             \State $\hat{k} \gets k$
%         \EndIf
        
%     \EndFor
%     \State $\hat{C} \gets \emptyset$
%     \State $lastCP \gets m$
    
%     \For{$k = \hat{k},\ldots,1$} \Comment{Retrieve change point set}
%         \State $lastCP \gets cpMat[k, lastCP]$
%         \State $\hat{C} \gets \hat{C}\cup\{ lastCP \}$
%     \EndFor
    
%     \Return $\hat{k}, \hat{C}$ 
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}
%%% -------------------------------------------------------------
\subsection*{Finite state Markov chain}

Let $A=\{a_1,\dotsc, a_d\}$ be a finite set and for each $\ell\in\N$ denote by $\F_{\ell}$ the distribution of a stationary Markov chain on the finite samples of length  $\ell$. That is,  $\F_{\ell}$ are the distributions over $A^\ell$ given by 
\[
p(x_{1:\ell})= \mu(x_1)\prod_{i=2}^{\ell} q(x_i|x_{i-1})\,, \qquad x_{1:\ell}\in A^\ell
\]
for some stationary distribution $\mu$ and some transition probability matrix $q\in [0,1]^{d\times d}$. We assume the Markov chain defined by $\mu$ and $q$ is irreducible and aperiodic.  Observe that in this case the variables inside each block in the model given by  \eqref{prob} are not independent. 

% Then the log-likelihood function \eqref{likelihood} can be written, for $C\in\C$ and $\theta=( (\mu_1,q_1),\dots, (\mu_k,q_k))$ as 
% \begin{equation}
% \P_{(C,\theta)}(\bx) = \prod_{j=1}^{k} p_j(x_{(c_{j-1}+1):c_j}).
%  \end{equation}
 The log-likelihood for the sample $\{\bx^{(i)}\}_{i=1}^n$ in \eqref{log-likelihood} can be written as
 \begin{equation}
l(C;\bx) = \sum_{j=1}^{k} \sum_{i=1}^n
\log f_{\widehat \mu_j, \widehat q_j}\Bigl(x_{(c_{j-1}+1):c_j}^{(i)}\Bigr) \,,
\end{equation}
where $\widehat\mu_j$ and $\widehat q_j$ are the maximum likelihood estimators of the initial distributions and transition matrix of the Markov chain. For simplicity in the notation we write
\[
\sum_{i=1}^n
\log f_{\widehat \mu_j, \widehat q_j}\Bigl(x_{(c_{j-1}+1):c_j}^{(i)}\Bigr) = \log f_{\widehat \mu_j, \widehat q_j}\Bigl(x_{(c_{j-1}+1):c_j}^{(1:n)}\Bigr)
\]
and then we only have a sum on the number of segments. 
It can be seen that the maximum likelihood estimators for the interval $I_j=(c_{j-1}+1, c_j)$  are given by  
\[
\widehat\mu_j = \frac{N_{c_{j-1}+1}(a)}{n} 
\]
and
\[
\widehat q_j = \frac{N_{I_j}(b,a)}{N_{I_j}(b,\cdot)}
\]
with 
\begin{equation}
 \begin{split}
     N_{c_{j-1}+1}(a) \;&=\; \sum_{i=1}^n\mathbf{1}\{x^{(i)}_{c_{j-1}+1}=a\}\\
     N_{I_j}(b,a) \;&=\; \sum_{i=1}^n \sum_{v=c_{j-1}+1}^{c_j-1}  \mathbf{1}\{x^{(i)}_v=b,x^{(i)}_v=a \}\\
     N_{I_j}(b,\cdot) \;&=\; \sum_{a\in A}   N_{I_j}(b,a)\,.
\end{split}
 \end{equation}
Then we have
\begin{equation}
\begin{split}
 \log f_{\widehat \mu_j, \widehat q_j}\Bigl(x_{(c_{j-1}+1):c_j}^{(1:n)}\Bigr) = &
\sum_{a\in A} N_{c_{j-1}+1}(a)\log \frac{N_{c_{j-1}+1}(a)}{n} \\
&+ \sum_{a,b\in A} N_{I_j}(b,a) \log \frac{N_{I_j}(b,a)}{N_{I_j}(b,\cdot)}
\end{split}
\end{equation}
As the samples are independent, by the Law of Large Numbers we have that 
\begin{equation}
\begin{split}
\frac1n  \log f_{\widehat \mu_j, \widehat q_j}\Bigl(x_{(c_{j-1}+1):c_j}^{(1:n)}\Bigr) \;\rightarrow \; &\sum_{a\in A} \mu_{i_j}(a) \log \mu_{i_j}(a) \\
&+ \sum_{a,b\in A} (|I_j|-1) \bar q_{I_j}(b,a) \log \bar q_{I_j}(a|b)\\
\end{split}
\end{equation}
% y the consistency of the estimators $\widehat\mu$ and $\widehat q$ we have that 
% %Ergodic Theorem \citep[Theorems I.3.1 and I.3.2]{shields1996} we have that 
% \begin{equation*}
% \begin{split}
% \frac1n l(C;\bx) \;\to\;&\sum_{j=1}^{k} 
% f_{\mu_{i_j}, \bar q_j}\Bigl(x_{(c_{j-1}+1):c_j}^{(1:n)}\Bigr)\\
% &\sum_{a\in A} \bar\mu_{j_i}(a) \log \bar\mu_{j_i}(a) + \sum_{a,b\in A} (|I_j|-1) \bar q_{I_j}(b,a) \log \bar q_{I_j}(a|b)\\
% & := \; l^*(C)\\
% \end{split}
% \end{equation*}
with $\mu_{i_j} = \mu_{r}$ if $i_j \in (c_{r-1}^*+1):c_r^*$, and 
\begin{equation}
    \begin{split}
         \bar q_{I_j}(a|b) \;&=\; \sum_{i=1}^{k^*}  \frac{|I_j\cap I^*_i|}{|I_j|} q_i(a|b) \qquad b,a\in A\\
          \bar q_{I_j}(b,a) \;&=\; \sum_{i=1}^{k^*}  \frac{|I_j\cap I^*_i|}{|I_j|} \mu_i(b)q_i(a|b) \qquad b,a\in A
    \end{split}
\end{equation}
%  \begin{equation}
%  l(C;\bx) = \sum_{j=1}^{k} \sum_{a\in A} N_{c_{j-1}+1}(a)\log \frac{N_{c_{j-1}+1}(a)}{n} + \sum_{a,b\in A} N_{I_j}(b,a) \log \frac{N_{I_j}(b,a)}{N_{I_j}(b,\cdot)}\,,
%  \end{equation}
%  where for any $v\in\{1,\dots,m\}$ and any block $I_j$
%  \begin{equation}
%  \begin{split}
%      N_{v}(a) \;&=\; \sum_{i=1}^n\mathbf{1}\{x^{(i)}_v=a\}\\
%      N_{I_j}(b,a) \;&=\; \sum_{i=1}^n \sum_{v=c_{j-1}+1}^{c_j-1}  \mathbf{1}\{x^{(i)}_v=b,x^{(i)}_v=a \}\\
%      N_{I_j}(b,\cdot) \;&=\; \sum_{a\in A}   N_{I_j}(b,a)\,.
% \end{split}
%  \end{equation}
To check (i) let $C\not\supseteq C^*$. 
 \begin{equation}
 l(C;\bx) = \sum_{j=1}^{k} \sum_{a\in A} N_{c_{j-1}+1}(a)\log \frac{N_{c_{j-1}+1}(a)}{n} + \sum_{a,b\in A} N_{I_j}(b,a) \log \frac{N_{I_j}(b,a)}{N_{I_j}(b,\cdot)}\,,
 \end{equation}
 where for any $v\in\{1,\dots,m\}$ and any block $I_j$
 \begin{equation}
 \begin{split}
     N_{v}(a) \;&=\; \sum_{i=1}^n\mathbf{1}\{x^{(i)}_v=a\}\\
     N_{I_j}(b,a) \;&=\; \sum_{i=1}^n \sum_{v=c_{j-1}+1}^{c_j-1}  \mathbf{1}\{x^{(i)}_v=b,x^{(i)}_v=a \}\\
     N_{I_j}(b,\cdot) \;&=\; \sum_{a\in A}   N_{I_j}(b,a)\,.
\end{split}
 \end{equation}




By the Law of Large Numbers we have that 
\[
\frac{N_{c_{j-1}+1}(a)}n\log \frac{N_{c_{j-1}+1}(a)}{n}  \;\to\; \mu_{i_j}(a)
\]
for all $a\in A$, where $i_j = r$ if $c_{j-1}+1 \in (c_{r-1}^*+1):c_r^*$. 
On the other hand 
\[
N_{I_j}(b,a) \log \frac{N_{I_j}(b,a)}{N_{I_j}(b,\cdot)} \;\to\; (|I_j|-1) \bar q_{I_j}(b,a) \log \bar q_{I_j}(a|b)
\]
for all $a,b\in A$, where 
\begin{equation}
    \begin{split}
         \bar q_{I_j}(b,a) \;=\; \sum_{i=1}^{k^*}  \frac{|I_j\cap I^*_i|}{|I_j|} q_i(a|b) \qquad b,a\in A\,.
    \end{split}
\end{equation}
%Then there exists an interval $(c_{i-1}+1):c_{i}$, $i\geq 1$,  containing a change point $c^*_j\in C^*$, $1\leq j\leq k-1$. 
By the consistency of the estimators $\widehat\mu$ and $\widehat q$ we have that 
%Ergodic Theorem \citep[Theorems I.3.1 and I.3.2]{shields1996} we have that 
\begin{equation*}
\begin{split}
\frac1n l(C;\bx) \;\to\;&\sum_{j=1}^{k} 
f_{\mu_{i_j}, \bar q_j}\Bigl(x_{(c_{j-1}+1):c_j}^{(1:n)}\Bigr)\\
&\sum_{a\in A} \bar\mu_{j_i}(a) \log \bar\mu_{j_i}(a) + \sum_{a,b\in A} (|I_j|-1) \bar q_{I_j}(b,a) \log \bar q_{I_j}(a|b)\\
& := \; l^*(C)\\
\end{split}
\end{equation*}
with $\mu_{i_j} = \mu_{r}$ if $i_j \in (c_{r-1}^*+1):c_r^*$, and 
\begin{equation*}
\begin{split}
  \bar q_{I_j}(a|b) \;=\; \sum_{i=1}^{k^*}  \frac{|I_j\cap I^*_i|}{|I_j|} q_i(a|b) \qquad b,a\in A\,. \quad {\color{blue}verificar!}  
\end{split}    
\end{equation*}
Moreover we have that 
\begin{equation}
\begin{split}
l^*(C) - l^*(C^*) &\;= \;   \sum_{j=1}^{k} \sum_{i=1}^{k^*} |I_j\cap I^*_i|  \sum_{a\in A}  p_i(a) \log \bar p_{I_j}(a)  -  \sum_{i=1}^{k^*} |I^*_i|  \sum_{a\in A}  p_i(a) \log p_i(a)\\
 &=  \; \sum_{j=1}^{k} \sum_{i=1}^{k^*} |I_j\cap I^*_i|  \sum_{a\in A}  p_i(a) \log \frac{\bar p_{I_j}(a)}{p_i(a)}\\
 &< \;0
\end{split}
\end{equation}
unless $\bar p_{I_j} = p_i$ for all $i$ and $j$ with $|I_j\cap I^*_i|\neq\emptyset$. But this can only happen if $C\supseteq C^*$, what is a contradiction. 

To verify hypothesis (ii) observe that for any $C\supseteq C^*$
\begin{equation*}
 \begin{split}
 l(C;\bx)  - l(C^*;\bx) \;&=\; \sum_{j=1}^{k} \sum_{a\in A} N_{I_j}(a) \log \frac{N_{I_j}(a)}{n|I_j|} - \sum_{j=1}^{k^*} \sum_{a\in A} N_{I_j^*}(a) \log \frac{N_{I_j^*}(a)}{n|I_j^*|}\\
 &\leq \sum_{j=1}^{k} \sum_{a\in A} N_{I_j}(a) \log \frac{N_{I_j}(a)}{n|I_j|} - \sum_{j=1}^{k^*}  \sum_{a\in A}  N_{I_j^*}(a)  \log p_j(a)\,,
\end{split}
\end{equation*}
where the last inequality follows because $N_{I_j^*}(a)/n|I_j^*|$ are the maximum likelihood estimators for $p_j(a)$.  As $C\supseteq C^*$ we have that any interval $I_i^*$ contains one or more intervals $I_j$, and 
\[
N_{I_i^*}(a) \; = \; \sum_{i: I_i\subseteq I_j^*}N_{I_j}(a) \qquad\text{ for all }a\in A\,.
\]
Then we can write the difference above as
\begin{equation*}
\begin{split}
\sum_{j=1}^{k} \sum_{a\in A} N_{I_j}(a) \log \frac{N_{I_j}(a)/n|I_j|}{p_{i_j}(a)}
\end{split}
\end{equation*}
where $i_j$ is the corresponding index in $C^*$. Therefore we obtain that 
\begin{equation*}
\begin{split}
l(C;\bx)  - l(C^*;\bx) \;&\leq\; \sum_{j=1}^{k}  n |I_j| D(\hat p_j(a) ; p_{i_j}(a))\,.
\end{split}
\end{equation*}
By a well-known inequality we have that 
\[
D(\hat p_j(a) ; p_{i_j}(a)) \;\leq\; \sum_{a\in A} \frac{|\hat p_j(a) - p_j(a)|^2}{p_j(a)}\,.
 \]
 As the difference $N_{I_j}(a) - n|I_j|p_j(a)$ can be written a sum of zero-mean independent random variables with finite variance, we have, by the Law of the Iterated Logarithm that 
\[
|\hat p_j(a) - p_j(a)| \;\leq\; \sqrt{\frac{c\log\log n|I_j|}{n|I_j|}}
\]
for a given constant $c$, eventually almost surely as $n\to\infty$. Then, for any $\delta>0$
we have that 
\[
|\hat p_j(a) - p_j(a)| \;\leq\; \sqrt{\frac{\delta \log n|I_j|}{n|I_j|}}
\]
eventually almost surely as $n\to\infty$.
Finally we obtain that 
\begin{equation*}
    \begin{split}
    l(C;\bx)  - l(C^*;\bx) \;&\leq\;  \frac{k\delta}{p_{\min}} \log n\;\leq\; \frac{m\delta}{p_{\min}}\log n \,,
    \end{split}
\end{equation*}
with $p_{\min} = \min\{p_j(a) \colon p_j(a)>0,  j=1,\dots,k^*, a\in A\}$.  On the other hand it is ease to see that 
\[
  l(C;\bx)  - l(C^*;\bx) \;\geq\; 0
\]
for any $C\supseteq C^*$. Then, hypothesis (ii) holds for $v(n)=c\log n$, for any $c>0$. 
